Evaluating Code Readability and Legibility: An Examination of Human-centric Studies

Reading code is an essential activity in software maintenance and evolution. Several studies with human subjects have investigated how different factors, such as the employed programming constructs and naming conventions, can impact code readability, i.e., what makes a program easier or harder to read and apprehend by developers, and code legibility, i.e., what influences the ease of identifying elements of a program. These studies evaluate readability and legibility by means of different comprehension tasks and response variables. In this paper, we examine these tasks and variables in studies that compare programming constructs, coding idioms, naming conventions, and formatting guidelines, e.g., recursive vs. iterative code. To that end, we have conducted a systematic literature review where we found 54 relevant papers. Most of these studies evaluate code readability and legibility by measuring the correctness of the subjects' results (83.3%) or simply asking their opinions (55.6%). Some studies (16.7%) rely exclusively on the latter variable.There are still few studies that monitor subjects' physical signs, such as brain activation regions (5%). Moreover, our study shows that some variables are multi-faceted. For instance, correctness can be measured as the ability to predict the output of a program, answer questions about its behavior, or recall parts of it. These results make it clear that different evaluation approaches require different competencies from subjects, e.g., tracing the program vs. summarizing its goal vs. memorizing its text. To assist researchers in the design of new studies and improve our comprehension of existing ones, we model program comprehension as a learning activity by adapting a preexisting learning taxonomy. This adaptation indicates that some competencies are often exercised in these evaluations whereas others are rarely targeted.

==> unused-content.tex <==
\begin{table}[h]
    \caption{Exclusion criteria.}
    \label{tab:exclusion-criteria}
    \centering
    \begin{tabular}{l p{0.41\textwidth}}
        \toprule
        ID & Description \\
        \midrule
        EC1 & Out of primary scope: The study is not primarily related to source code comprehension and readability, does not involve any kind of comparison of program characteristics, neither direct nor indirect, or is clearly irrelevant to our research questions. For instance, a study focusing on system architecture, high-level design, documentation, or dependencies between system parts (higher-level issues) is excluded. \\
        EC2 & The study is not a full paper (e.g. master dissertations, doctoral theses, course completion monographs, short papers) or is not written in English. As a rule of thumb, we consider that full papers must be at least 5 pages long. \\
        EC3 & The study is about readability metrics without experimental evaluation. \\
        EC4 & The study is about program understanding aids, such as visualizations or other forms of analysis or sensory aids (e.g. graphs, trace-based execution, code summarization, specification mining, reverse engineering). \\
        EC5 & The study has a focus on accessibility, e.g., study focusing on people with visual impairments or neurodiverse developers (as Autism Spectrum Disorder). \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Inclusion criteria.}
    \label{tab:inclusion-criteria}
    \centering
    \begin{tabular}{l p{0.41\textwidth}}
        \toprule
        ID & Description \\
        \midrule
        IC1 & Scope: The study must be primarily related to the topics of code readability, legibility, understandability, or hard-to-understand code. \\
        IC2 & Methodology: The study must be/contain at least one empirical study, such as controlled experiment, quasi-experiment, case study, or survey. \\
        IC3 & Comparison: The study must compare alternative programming language constructs, coding idioms, or coding styles. The study may compare those elements \textit{directly}, e.g., controlled experiments measuring the performance of subjects in code reading tasks, or \textit{indirectly}, e.g., case studies collecting metrics related to these elements and validating them against some criteria (e.g., expert judgement) to assess readability. \\
        IC4 & Granularity: The study must target fine-grained program elements and low-level/limited-scope programming activities. Not design or comments, but implementation. \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[t]
{\scriptsize
\caption{Study quality assessment questions. The possible answers for each question are yes (1)/partially (0.5)/no (0).}
    \label{tab:quality-assessment-questions}
    \centering
    \begin{tabular}{@{} l p{0.43\textwidth} @{}}
        \toprule
        \# & Question \\
        \midrule
        \multicolumn{2}{@{}l@{}}{Questions about design} \\
        1 & Are the aims clearly stated? \\
        2 & Are the independent variables adequately defined? \\
        3 & Are the response variables adequately defined? \\
        \midrule
        \multicolumn{2}{@{}l@{}}{Questions about analysis and rigor} \\
        4 & Are the data collection methods adequately described? \\
        %5 & Are the study participants or observational units adequately described? \\
        5 & Are the study participants adequately described? \\
        6 & Were the collected data adequately described? \\
        7 & Did the study employ statistical methods to analyze the data? \\
        \midrule
        \multicolumn{2}{@{}l@{}}{Questions about conclusion} \\
        %8 & Is there a clear statement of findings, i.e., are all study questions answered? \\
        8 & Is there a clear statement of findings? \\
        9 & Do the researchers explain the threats to the study validity? \\
        \bottomrule
    \end{tabular}
    }
\end{table}

\noindent\textit{General study removal.}
Additionally, there were three special cases where we removed documents, which we describe as follows. First, some documents were removed during the triage or the initial section steps that were duplicates. We performed an automatic checking for that, but some documents had different names, yet were referring to the same thing. Second, we also removed some documents that were not research documents, such as proceedings. Finally, there were some documents that were actually removed in the initial selection, when the inclusion criteria is applied, but because of some exclusion criterion. An example is about papers written in a language other than English. In the triage, we read the title and abstract, and we found those in English, but when actually finding the paper in the initial selection step, we discovered that the paper was not in English.

\todo{Which code elements can affect in comprehension?}
The code features are factors that can affect the program understandability.  Buse and Weimer \cite{Buse2010}, Posnett et al \cite{Posnett2011}, Dorn \cite{dorn}, and Scalabrino \cite{Scalabrino2019} proposed metrics to measure code comprehension through code features, for example, \#identifiers, \#operators, indentation, loops. In this context, some studies investigate how these features affect the code comprehension. For example, these papers compare how to construct an identifier \cite{Schankin2018}\cite{Lawrie2007}\cite{Avidan2017}\cite{Butler2010}, regular and non-regular code \cite{Jbara2017}\cite{Jbara2014b}, code patterns \cite{Gopstein2017}\cite{Yeh2017}\cite{Medeiros2019}, or how use pre-processors \cite{Schulze2013}\cite{Malaquias2017}.

%However, there are different types of tasks and evaluation methods to do in an experiment of code comprehension. Siegmund and Schumann \cite{siegmund2015confounding}, identify relevant confounding parameters and select appropriate techniques to control their influence. In view, the importance given by the academy in recent years to the subject of code understanding, it is necessary to explore which experimental methods are available and how to use it.

%In this sense, the readability of the code can impact the overall quality of a software, since it can not only hinder the understanding of the code but can also lead to the implementation of potential errors according to Mynatt \cite{mynatt1984effect}. Then there are methods to assess Readability, which according to Tashtoush et al. \cite{tashtoush2013impact}, are one of the needs arising from advances in programming languages and from increasing the complexity of programs. The author states that in linguistics the subject of readability has been studied for a long time, which provided for the creation of a measurement model. However, these statistical models explore the correlation between text resources and the level of readability perceived by the reader, by nature these models are prone to errors.

%However, the work of Almeida et al. \cite{de2003best} states that legibility is essential for maintaining the code. In the work, the authors expose eight items that can be checked in the code to obtain legibility. Another interesting work on readability is that of Moonen \cite{moonen2003exploring}, in which the author states that the readability of the software is an important aspect because they can make the software easier to maintain. The authors Reddivari and Kotapalli in their work \cite{reddivari2017use} reinforce the idea that readability is an important factor in understanding code.



%In the remainder of this section, we explain the activities listed in \autoref{tab:study-analysis-activities} in a bit more detail.

% \textbf{Adapt, Apply, and Implement.}
% The Adapt activity is about the modification of a solution to fit in a given context, while Apply is about changing a context so that an existing solution fits in it. Furthermore, Apply is different from Implement because Apply is about using existing solutions, while Implement is about coding a solution given a description.

% \textbf{Debug, Inspect, and Trace.}
% The Debug activity is about examining the code to search for a bug and possibly fixing it, while Inspect is only about scanning the code for general purposes. Moreover, Inspect involves checking properties about the static structure of a program while Trace pertains to program behavior, i.e., what it does at run time.

% \textbf{Design, Model, and Present.}
% The Design activity is different from the Model activity because the subject must build the solution from a problem, while Model has a solution as a basis. The Model activity is different from the Present activity because the input is a model (a solution description, for example) while the input to Present is the source code.

% \textbf{Present, Relate, and Inspect.}
% The Present activity is different from Relate because the subject must explain the objective of a program, while Relate must compare with similar ones. Also, Present is different from Inspect because the subject must explain the code proposal, while Inspect makes a query to code.

% \textbf{Recognize, Memorize, and Relate.}
% The Recognize activity requires that the subject remembers a concept or code structure obtained before the task, while in Memorize the subject must remember elements or code structures from a part of the task. Furthermore, Recognize requires prior knowledge whereas Relate does not.

% \textbf{Debug and Refactor.}
% Both Debug and Refactor activities involve changing a program.
% The Debug activity starts from the assumption that a given program does not behave according to its specification, and aims to identify and possibly fix the root cause of this deviation. Refactor, on the other hand, starts from the assumption that a given program behaves according to its specification, and aims to modify only non-functional properties.




% \section{Related Works}

% The works that are related to ours are studies that analyze how code comprehension is evaluated, and systematic reviews or surveys on code comprehension. In this context, Siegmund\cite{siegmund2016} presented a list of methods to evaluate comprehension such as think-aloud protocols, memorization, comprehension tasks, and neuro-imaging techniques. In contrast to our work, this list is not based on a literature survey of comprehension experiments. Furthermore, our work presents more methods, their multi-facets, and types of response variables. 

% There are many literature reviews about empirical studies in software engineering (SE). For example, Sjøberg et al.\cite{sjoberg2005} reported a survey that characterized quantitatively the controlled experiments in SE; and Kampenes et al.\cite{kampenes2009} reported a systematic review of the literature to investigate the extent of randomization and quasi-experimentation in SE. These studies considered papers in the general context of SE, and not only about code comprehension. Otherwise, Schröter et al.\cite{schroter2017comprehending}, conducted a manual literature review to explore empirical studies on program comprehension at the International Conference on Program Comprehension (ICPC). They found which parts of the understanding of the program are being investigated, what are the terminologies used, and whether the research reports its threats to validity. They did not analyze how these studies evaluate code comprehension in experiments.

% Other literature reviews were aiming at experiment features. Kampenes et al \cite{kampenes2007} reported a systematic review that investigated the practice of effect size reporting, summarizes standardized effect sizes detected in the experiments. Dybå et al. \cite{dyba2006} reported a systematic review that performed a quantitative assessment of the statistical power of current experimental SE research. Likewise, Siegmund et al. \cite{siegmund2015confounding}  presented a catalog of confounding parameters for comprehension experiments based on a literature survey, including applied measurement and control techniques. Similar to our work, these studies investigated the experiment design of primary studies, but in the perspective of effect sizes and inference models of experiments, while our work is interested in practices performed by subjects and their evaluation methods. In addition, the two first surveys considering works beyond the code comprehension.

% In summary, our study differs from the others in that it conducted research following the steps of a systematic literature review. We aimed to identify in the literature how the studies centered on the human being evaluate if a certain approach is more readable or legible than another.


%This work is part of a larger initiative where we intend to identify an ideal set of constructs, idioms, and style guidelines that promote readability and legibility.

% To sum up, our contributions are:

% \begin{itemize}[leftmargin=1.1em]
%     \item Definition of the terms ``readability'' and ``legibility'' in the context of Software Engineering.
%     \item An investigation of comprehension tasks and response variables involved in empirical studies where readability or legibility are evaluated.
%     \item Adapting a learning taxonomy to support an analysis of program comprehension tasks according to their required cognitive skills
% \end{itemize}

% The remaining of this paper is organized as follows. In \autoref{sec:code-readability-and-legibility} we present the concepts of legibility and readability that guided our study. The methodology used, as well as the steps and decisions taken, are presented in \autoref{sec:methodology}. \autoref{sec:results} presents the answers to our research questions, and the analysis of program comprehension as a learning activity is presented in \autoref{sec:program-comprehension-as-a-learning-activity}. Finally, we discuss the threats to validity in \autoref{sec:threats-to-validity} and present final remarks in \autoref{sec:conclusion}.






